Counterfactual Explanation Policies in RL

As Reinforcement Learning (RL) agents are increasingly employed in diverse decision-making problems using reward preferences, it becomes important to ensure that policies learned by these frameworks in mapping observations to a probability distribution of the possible actions are explainable. However, there is little to no work in the systematic understanding of these complex policies in a contrastive manner, i.e., what minimal changes to the policy would improve/worsen its performance to a desired level. In this work, we present COUNTERPOL, the first framework to analyze RL policies using counterfactual explanations in the form of minimal changes to the policy that lead to the desired outcome. We do so by incorporating counterfactuals in supervised learning in RL with the target outcome regulated using desired return. We establish a theoretical connection between Counterpol and widely used trust region-based policy optimization methods in RL. Extensive empirical analysis shows the efficacy of COUNTERPOL in generating explanations for (un)learning skills while keeping close to the original policy. Our results on five different RL environments with diverse state and action spaces demonstrate the utility of counterfactual explanations, paving the way for new frontiers in designing and developing counterfactual policies.

==> 000questions.tex <==
This document contains questions that reviewers can raise:
1. How are these counterfactual policies different from policies obtained using causal analysis?
2. Why would one want to derive counterfactual policies this way?
3. What is the use of counterfactual policies?
4. How does this compare with just applying PPO with plus/minus rewards and training until the target return has been hit? Can't we find counterfactuals using such a technique? And what about the insights gotten through them?

